A new look inside Planetary Nebula LoTr 5: A long-period binary with hints of a possible third component

LoTr 5 is a planetary nebula with an unusual long-period binary central star. As far as we know, the pair consists of a rapidly rotating G-type star and a hot star, which is responsible for the ionization of the nebula. The rotation period of the G-type star is 5.95 days and the orbital period of the binary is now known to be $\sim$2700 days, one of the longest in central star of planetary nebulae. The spectrum of the G central star shows a complex H$\alpha$ double-peaked profile which varies with very short time scales, also reported in other central stars of planetary nebulae and whose origin is still unknown. We present new radial velocity observations of the central star which allow us to confirm the orbital period for the long-period binary and discuss the possibility of a third component in the system at $\sim$129 days to the G star. This is complemented with the analysis of archival light curves from SuperWASP, ASAS and OMC. From the spectral fitting of the G-type star, we obtain a effective temperature of $T_{\rm eff}$ = 5410$\pm$250 K and surface gravity of $\log g$ = 2.7$\pm$0.5, consistent with both giant and subgiant stars. We also present a detailed analysis of the H$\alpha$ double-peaked profile and conclude that it does not present correlation with the rotation period and that the presence of an accretion disk via Roche lobe overflow is unlikely.

==> sec3_1.tex <==
%==============================
\subsection{Archival light curves analysis}
%==============================
\label{sec:lc}





\begin{figure}
\includegraphics[width=\columnwidth]{LC_SuperWASP_Periodogram_Residuals.pdf}
\caption{Top: Periodogram of the residuals of the superWASP data after removing the $\sim$5.95~days signal. The $\sim129$~days peak is also marked with a vertical dashed line. Bottom: Light curve residuals after removing the$\sim$5.95~days signal and phase-folded with the 129 days periodicity}
\label{fig:superwasp_residuals}
\end{figure}



In Fig.~\ref{fig:LCperiodograms}, we show the Lomb-Scargle periodograms of the three photometric datasets. In the case of superWASP and ASAS, we find a significant peak at $P\sim5.95$~days (assumed to be the rotation period of the (sub)giant star, see Sect.~\ref{sec:introduction}). We can model this signal with a simple sinusoid to estimate the period and amplitude of the variations independently in each dataset. We left the period to vary freely between 0 and 10 days in all cases and found: $P_{\rm WASP} = 5.95092\pm0.00062$~days, $P_{\rm ASAS} = 5.9409\pm0.0021$~days, $P_{\rm OMC} = 5.94579\pm0.00012$~days. Fig.~\ref{fig:activity_wasp} shows the phase-folded light curves of the three datasets with these periods. The corresponding semi-amplitudes are $A_{\rm WASP}=12.93\pm0.52$~mmag, $A_{\rm ASAS}=20.2\pm2.9$~mmag, $A_{\rm OMC}=18.12\pm0.41$~mmag. These results, \textcolor{red}{together with the date range of the data,} are summarized in Table ~\ref{Table:results_LCs}.  \textcolor{red}{The amplitude clearly varies from one lightcurve to each others. This might be due to the different timespan of the datasets covering different time ranges of the stellar cycle (i.e., different amount of star spots). In the case of SuperWASP, the data were taken in a short time span (only four months), so the stellar spots are steady along this time. On contrary, in the case of ASAS and OMC, where the data are spread over years, the amplitude due to star sports is diluted because we are probably mixing periods of stellar maxima and stellar minima}.


If we now remove this signal from the SuperWASP dataset (the most precise one) and calculate the periodogram of the residuals, other prominent (although non-significant) peaks appear (see Fig.~\ref{fig:superwasp_residuals}, top panel). In particular, we want to highlight the peak at $\sim129$~days. This is relevant because it also appears in the radial velocity analysis (see Sect.~\ref{sec:129days}). The phase-folded light curve with that period is shown in Fig.~\ref{fig:superwasp_residuals}, bottom panel. The origin of this peak will be discussed in detail in Sect.~\ref{sec:radial_velocity} together with the $\sim5.95$~days periodicity.



